Exponential Segregation in a Two-Dimensional Schelling Model with Tolerant Individuals

We prove that the two-dimensional Schelling segregation model yields monochromatic regions of size exponential in the area of individuals' neighborhoods, provided that the tolerance parameter is a constant strictly less than 1/2 but sufficiently close to it. Our analysis makes use of a connection with the first-passage percolation model from the theory of stochastic processes.

==> geometry.tex <==
\section{Persistence of Monochromatic Balls}

Lemma \ref{lem:big.ball} bounds the probability that a given node $x$ will be contained in a large monochromatic region, at \emph{some} time $t$.  However, our main result requires that $x$ be contained in a large monochromatic region in the final configuration $\sigma_T$.  In this section, we show that a sufficiently large monochromatic region will persist until time $T$.
%
Given a node $x$, write $B_R(x)$ for the set of nodes $y$ with $||x-y||_2 \leq R$, where $||x-y||_2$ denotes Euclidean distance.

\begin{lemma}
\label{lem:ball.persists}
Fix $\epsilon > 0$ and take $w$ sufficiently large.  Suppose $B_R(x)$ is monochromatic in configuration $\sigma_t$, where $R \geq w^3$.  Then for any $t' > t$, $B_R(x)$ is monochromatic in $\sigma_{t'}$.
\end{lemma}
\begin{proof}
It suffices to show that every node in $B_R(x)$ would be happy even if all nodes outside $B_2(R)$ take the opposite spin.  We will prove this by establishing that, for every $v \in B_R(x)$, at least $(\frac{1 - \epsilon}{2})(2w+1)^2$ neighbors of $v$ lie inside $B_R(x)$.  

Consider a point $v$ lying on the boundary of $B_R(x)$.  Consider the line $L$ tangent to the boundary of $B_R(x)$ at $v$.  By symmetry, precisely half of the neighbors of $v$ (excluding those that lie on $L$) lie on either side of line $L$.  It therefore suffices to show that the number of neighbors of $v$ that lie strictly between $L$ and the boundary of $B_R(x)$ is less than $\frac{\epsilon}{2}(2w+1)^2$.  

Since the boundary of $B_R(x)$ has curvature $R^{-1} \leq w^{-3}$, and the neighborhood of $v$ is contained within a ball of radius $\theta(w)$, the boundary and $L$ differ in slope by at most $\theta(w^{-2})$ within the neighborhood of $v$.  The area between $v$ and $B_R(x)$ is therefore contained within the area between $L$ and line $L$ shifted orthogonally by a distance of $\theta(1/w)$, again because the neighborhood of $v$ is contained within a ball of radius $\theta(w)$.  If $w$ is sufficiently large, then for any point $x$ in that area, the box $x + [\pm 0.5, \pm 0.5]$ must intersect line $L$.  Since any line intersects at most $\theta(w)$ such boxes, we conclude that at most $\theta(w)$ vertices lie strictly between $L$ and the boundary of $B_R(x)$.  This is less than the required $\frac{\epsilon}{2}(2w+1)^2$, for $w$ sufficiently large.
%This implies, again because of the neighborhood of $v$ is contained within a ball of radius $\theta(w)$, that each point of $L$ is within distance $O(1/w)$ of $B_2(R)$.  
\end{proof}

